LZMidi: Compression-Based Symbolic Music Generation

Recent advances in symbolic music generation primarily rely on deep learning models such as Transformers, GANs, and diffusion models. While these approaches achieve high-quality results, they require substantial computational resources, limiting their scalability. We introduce LZMidi, a lightweight symbolic music generation framework based on a Lempel-Ziv (LZ78)-induced sequential probability assignment (SPA). By leveraging the discrete and sequential structure of MIDI data, our approach enables efficient music generation on standard CPUs with minimal training and inference costs. Theoretically, we establish universal convergence guarantees for our approach, underscoring its reliability and robustness. Compared to state-of-the-art diffusion models, LZMidi achieves competitive Frechet Audio Distance (FAD), Wasserstein Distance (WD), and Kullback-Leibler (KL) scores, while significantly reducing computational overhead - up to 30x faster training and 300x faster generation. Our results position LZMidi as a significant advancement in compression-based learning, highlighting how universal compression techniques can efficiently model and generate structured sequential data, such as symbolic music, with practical scalability and theoretical rigor.

==> gpt_feedback.tex <==
Here's a careful, rigorous review of your paper, framed as feedback from an ISIT Workshop reviewer and from the perspective of a potential submission to ICML/NeurIPS workshops. The feedback is structured to clearly indicate what's currently strong, what could be improved, and concrete suggestions for enhancing the theoretical and empirical aspects of your work:

---

## ISIT Workshop Reviewer Feedback

### **Strengths:**
- **Relevant Theme:** Clearly aligned with the workshop’s focus on "Compress to Learn" by leveraging compression principles directly for symbolic music generation.
- **Computational Efficiency:** Demonstrates significant computational savings compared to deep learning methods, aligning well with the workshop’s emphasis on efficient neural compression and practical resource constraints.
- **Clear Motivation:** The work successfully identifies inefficiencies in current deep learning methods (particularly diffusion models) and positions compression-based techniques as viable, scalable alternatives.
- **Theoretical Contributions:** Clearly stated universal convergence guarantees provide solid theoretical grounding.

### **Areas for Improvement:**
- **Clarifying Metric Choice:** While the motivation behind using Wasserstein Distance is now clearer, it remains important to explicitly discuss why Wasserstein is more suitable than other simpler distributional metrics (e.g., histogram distances), particularly within the context of symbolic data versus audio embeddings.
- **Explicit Baseline Clarification:** It's helpful you've clarified your D3PM baseline’s training constraints. Clearly highlight earlier why you independently trained your baseline instead of using published results due to differences in sequence length (256 vs. 1024 tokens). Emphasize this clearly and early in the paper.
- **Use of the Symbol '1':** Provide deeper intuition or empirical evidence explaining why explicitly representing note continuation ('1') leads to superior performance. A brief experiment or a footnote with a hypothesis on this would be helpful.
- **Removing Implementation Details:** Your description of metric implementations is still somewhat detailed. Move very detailed computation steps to supplementary material or online repositories, keeping the paper concise and focused.

### **Suggestions to Address Above Points:**
- Clearly state in the main paper why the Wasserstein distance was specifically chosen over other simpler distributional metrics (e.g., histogram-based metrics).
- Clearly state earlier in your experimental section why you independently trained the baseline D3PM due to differences in training sequence length and hardware constraints.
- Provide either a short empirical ablation or clear theoretical intuition in an appendix section discussing the impact and necessity of the continuation symbol ('1').

---

## ICML/NeurIPS Workshop Reviewer Feedback (More Rigorous Lens):

### **Strengths:**
- Your paper effectively positions compression-based methods within the modern generative modeling landscape dominated by diffusion and transformer models.
- Empirical results clearly highlight significant computational gains (training and inference time) compared to deep learning baselines.
- Theoretical underpinning with universal convergence guarantees significantly strengthens the paper, adding to both practical and theoretical appeal.

### **Key Points of Critique and Suggestions for Improvement:**

#### **(1) Empirical Comparisons:**
- **Expanded Baseline Comparisons:**  
  Given that your baseline diffusion model (D3PM) was only partially trained due to computational limitations, including results of the fully-trained model in an appendix with clear caveats is valuable. However, explicitly highlight that sequence lengths differ (1024 tokens in the original work vs. 256 in yours), making direct comparison difficult. Provide a succinct table in the appendix clearly stating this difference to prevent confusion.

#### **(2) Theoretical Strengthening:**
- **Finite Sample Analysis:**  
  Your convergence theorem (Theorem III.1) relies on asymptotic conditions (m → ∞). An additional finite-sample analysis (either theoretically or empirically through simulation) could significantly strengthen relevance, clearly illustrating how fast LZMidi converges to the true distribution as training size grows practically.
  
- **Theoretical Justification of Symbol '1':**  
  Clarify further why explicitly representing the note-continuation symbol ('1') provides measurable gains. Provide theoretical intuition or simple illustrative examples (in the appendix) demonstrating why explicitly marking continuations might help LZ trees capture temporal structures more efficiently.

#### **(3) Terminology and Clarity Improvements:**
- **Ergodicity and Universality:**  
  Given expert feedback that ergodicity is primarily relevant as \( n \rightarrow \infty \), either clearly explain how your fixed-length experiments relate practically (finite-sample) to ergodic assumptions or simply omit ergodicity references entirely. If retained, emphasize explicitly that ergodicity is not critical in your finite-length experimental settings, keeping clarity for reviewers unfamiliar with information-theoretic nuances.

- **Compression Metrics Justification:**  
  Explicitly justify your chosen metrics (especially Wasserstein) in terms of their alignment with symbolic MIDI data and computational practicality (avoiding neural-network-based evaluation metrics during hyperparameter sweeps). Consider briefly mentioning the debate on compressor-based classification accuracy, as you've done previously, and emphasize your careful metric selection.

#### **(4) Additional Experiments or Analyses (Recommended for ICML/NeurIPS):**
- **Quantitative Ablation Study:**  
  Conduct a brief ablation showing the practical impact of the critical hyperparameters (`γ`, Top-K, temperature) on music quality. Clarify specifically which parameter contributes most significantly to performance.
  
- **Generalization & Transfer Learning:**  
  A brief empirical experiment evaluating how quickly your compression-based model adapts to new datasets or musical styles could significantly enhance your contribution, clearly highlighting how universal compression inherently generalizes or transfers to different symbolic datasets.

#### **(4) Broader Context and Impact:**
- **Sustainability & Efficiency:**  
  Briefly connect explicitly to broader efficiency and sustainability motivations. This resonates strongly with ICML/NeurIPS communities currently focused on reducing compute/carbon footprints of generative models.

#### **(4) FLOPS Analysis:**
- It's strongly recommended to include a concise but explicit side-by-side FLOPS comparison between your LZMidi and the ASD3PM baseline, clearly quantifying the computational advantages beyond CPU-time measurements.

---

### Suggested Relevant Workshops (ICML / NeurIPS):
- **NeurIPS/ICML Workshop on Efficient Methods in Machine Learning:**  
  Given your focus on computationally efficient alternatives to deep learning.
- **NeurIPS/ICML Workshop on Information-Theoretic Methods for Machine Learning:**  
  Directly relevant given your theoretical results around universal compression.
- **Workshop on Generative Models and Creative AI:**  
  Particularly relevant if you include more qualitative/human perceptual evaluation.
- **SustainML (Sustainability in ML Workshop):**  
  If you further highlight computational/resource efficiency as central motivation.

---

### Summary of Actionable Steps for Improvement:
- Add appendix table clarifying fully-trained D3PM comparison differences explicitly.
- Provide finite-sample theoretical intuition on universal convergence.
- Clarify ergodicity assumptions (or remove explicitly) as per expert advice.
- Provide brief theoretical or empirical justification for using symbol ‘1’.
- Clarify explicitly and justify the use of Wasserstein Distance.
- Include FLOPS analysis side-by-side for clear computational advantage.
- Consider additional short experiments on transfer/generalization.

These improvements would significantly enhance the submission, clearly aligning it with ISIT workshop goals and potentially making it attractive for future submissions to high-impact NeurIPS/ICML workshops.

==> next_steps.tex <==
Summary of Actionable Steps for Improvement:

Add appendix table clarifying fully-trained D3PM comparison differences explicitly.
Provide finite-sample theoretical intuition on universal convergence.
Clarify ergodicity assumptions (or remove explicitly) as per expert advice.
Provide brief theoretical or empirical justification for using symbol ‘1’.
Clarify explicitly and justify the use of Wasserstein Distance.
Include FLOPS analysis side-by-side for clear computational advantage.
Consider additional short experiments on transfer/generalization.
These improvements would significantly enhance the submission, clearly aligning it with ISIT workshop goals and potentially making it attractive for future submissions to high-impact NeurIPS/ICML workshops
